When Large Multimodal Models Confront Evolving Knowledge: Challenges and Explorations

Large Multimodal Models (LMMs) store vast amounts of pretrained knowledge but struggle to remain aligned with real-world updates, making it difficult to avoid capability degradation when acquiring evolving knowledge. Furthermore, most current work focuses on exploring static textual knowledge injection, neglecting dynamic multimodal evolving knowledge injection, leaving the potential of LMMs for multimodal knowledge injection as an open question. To address this, we first propose a pipeline to construct MMEVOKE, a benchmark for evaluating LMMs' ability in multimodal evolving knowledge injection. MMEVOKE contains 9,422 samples spanning 159 subtypes. Then, based on extensive experiments with MMEVOKE, we reveal challenges such as poor injection performance and capability degradation in existing knowledge injection methods through knowledge injection tests and general capability tests. Finally, to tackle these challenges, we introduce knowledge augmentation and knowledge retention methods, finding that knowledge-aware augmentation strengthens knowledge injection performance, and that Data Replay and MoE methods effectively mitigate capability degradation.

==> table/test.tex <==


% \begin{table*}[t!]
\begin{table*}[th]
\caption{\textbf{The results of LLaVA-v1.5 on general capability tests.} \tbf{First line} shows results of current methods in general capability tests; \tbf{Second line} shows the percentage of capability degradation or improvement of current methods compared to Vanilla. \hlredtabDB{Red value} indicates capability degradation, the darker the color, the more severe the degradation, and \hlredtabB{Green value} indicates capability improvement. \tbf{Ranking} includes average degree of degradation and degradation ranking. }






% \begin{table*}[htbp]
\centering
\resizebox{1.0\linewidth}{!}{
% \scalebox{0.55}{
\begin{tabular}{l|c c|c c|c c|c|c|c c|c c|c}
\toprule
\multirow{2.5}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{Comprehensive}} & \multicolumn{2}{c|}{\textbf{OCR}} & \multicolumn{2}{c|}{\textbf{Multidisciplinary}} & \multicolumn{1}{c|}{\textbf{Instruction}} & \multicolumn{1}{c|}{\textbf{Multi-Round}} & \multicolumn{2}{c|}{\textbf{Mathematical}} & \multicolumn{2}{c|}{\textbf{Hallucination}} & \multirow{2}{*}{\textbf{Ranking}} \\
\cmidrule{2-3}\cmidrule{4-5}\cmidrule{6-7} \cmidrule{8-8}\cmidrule{9-9}\cmidrule{10-11}\cmidrule{12-13}
& \textbf{MME} \daugshifted & \textbf{MMBench} \daugshifted & \textbf{SEED}\raisebox{1ex}{\tiny\textbf{B2P}} \daugshifted & \textbf{OCRBench} \daugshifted & \textbf{ScienceQA} \daugshifted & \textbf{MMMU} \daugshifted & \textbf{MIA-Bench} \daugshifted & \textbf{MMDU} \daugshifted & \textbf{MathVista} \daugshifted & \textbf{MathVision} \daugshifted & \textbf{POPE} \daugshifted & \textbf{HallusionBench} \daugshifted & \\

% \textbf{HallusionBench} 

% \multirow{2}{*}{7} 一个排名占两行

\midrule
Vanilla
& 1,865.56 & 64.60 & 38.78 & 30.80 & 69.83 & 28.60 & 66.33 & 26.37 & 25.50 & 13.16 & 86.87 & 21.76 & - \\
\midrule

Full-FT
& \ColorValue{48.71} & \ColorValue{18.08} & \ColorValue{18.93} & \ColorValue{8.77} 
& \ColorValue{3.87} & \ColorValue{15.38} & \ColorValue{61.93} & \ColorValue{50.59} 
& \ColorValue{3.14} & \ColorValue{9.27} & \ColorValue{14.56} & \ColorValue{57.40}  
&{\textbf{8}} \ColorValue{25.89}\\
\midrule

LoRA
& \ColorValue{33.88} & \ColorValue{16.61} & \ColorValue{22.07} & \ColorValue{16.56} 
& \ColorValue{5.23} & \ColorValue{25.17} & \ColorValue{55.28} & \ColorValue{48.05} 
& \ColorValue{9.02} & \ColorValue{2.51} & \ColorValue{14.85} & \ColorValue{59.65}
&{\textbf{7}} \ColorValue{25.74}\\
\midrule



\multicolumn{7}{l}{\fontsize{11}{13}\selectfont \textbf{Knowledge Augmentation for Text}} \\

{\begin{tabular}{l} Knowledge \\ Agnostic \end{tabular}}
& \ColorValue{21.36} & \ColorValue{11.83} & \ColorValue{16.09} & \ColorValue{14.94} 
& \ColorValue{1.36} & \ColorValue{22.38} & \ColorValue{65.48} & \ColorValue{59.76} 
& \ColorValue{12.55} & \ColorValue{37.77} & \ColorValue{6.30} & \ColorValue{62.13} 
&{\textbf{10}} \ColorValue{27.66}\\
\midrule



{\begin{tabular}{l} Knowledge \\ Aware (+3) \end{tabular}}
& \ColorValue{20.19} & \ColorValue{9.04} & \ua{2.27} & \ColorValue{12.99} 
& \ColorValue{1.26} & \ColorValue{6.29} & \ColorValue{64.36} & \ColorValue{60.03} 
& \ColorValue{7.45} & \ColorValue{27.51} & \ColorValue{15.76} & \ColorValue{26.03} 
&{\textbf{4}} \ColorValue{20.72}\\
\midrule


\multicolumn{7}{l}{\fontsize{11}{13}\selectfont \textbf{Knowledge Augmentation for Images}} \\

{\begin{tabular}{l} Knowledge \\ Agnostic \end{tabular}}
& \ColorValue{23.00} & \ColorValue{10.90} & \ColorValue{23.57} & \ColorValue{15.58} 
& \ColorValue{4.81} & \ColorValue{30.07} & \ColorValue{67.41} & \ColorValue{59.46} 
& \ColorValue{19.22} & \ColorValue{25.99} & \ColorValue{6.16} & \ColorValue{69.99} 
&{\textbf{11}} \ColorValue{29.68}\\
\midrule


{\begin{tabular}{l} Knowledge \\ Aware (+3) \end{tabular}}
& \ColorValue{33.07} & \ColorValue{16.08} & \ColorValue{6.68} & \ColorValue{18.83} 
& \ColorValue{4.17} & \ColorValue{5.59} & \ColorValue{72.85} & \ColorValue{59.73} 
& \ColorValue{19.61} & \ColorValue{38.22} & \ColorValue{11.17} & \ColorValue{36.95} &{\textbf{9}} \ColorValue{26.91}\\
\midrule




\multicolumn{7}{l}{\fontsize{11}{13}\selectfont \textbf{Knowledge Retention Methods}} \\

{Replay$_{\textbf{+10\%}}^{\textbf{Full-FT}}$} 
& \ColorValue{13.81} & \ColorValue{6.24} & \ColorValue{0.23} & \ColorValue{7.14} 
& \ColorValue{1.56} & \ua{1.75} & \ColorValue{22.81} & \ColorValue{31.40} 
& \ColorValue{4.31} & \ua{2.20} & \ColorValue{0.40} & \ColorValue{25.78} 
&{\textbf{3}}  \ColorValue{9.14}\\

\midrule
{Replay$_{\textbf{+10\%}}^{\textbf{LoRA}}$} 
& \ColorValue{11.51} & \ColorValue{6.38} & \ColorValue{1.13} & \ColorValue{7.14} 
& \ColorValue{1.52} & \ColorValue{0.35} & \ColorValue{6.03} & \ColorValue{26.77} 
& \ColorValue{1.18} & \ColorValue{0.23} & \ColorValue{1.65} & \ColorValue{17.74} 
& {\textbf{1}} \ColorValue{6.80}\\
\midrule

{EWC}
& \ColorValue{27.09} & \ColorValue{22.20} & \ColorValue{13.36} & \ColorValue{16.56} 
& \ColorValue{5.90} & \ColorValue{11.89} & \ColorValue{55.09} & \ColorValue{49.34} 
& \ColorValue{8.63} & \ColorValue{3.04} & \ColorValue{12.26} & \ColorValue{50.51} 
& {\textbf{5}} \ColorValue{22.99}\\
\midrule

{LwF}
& \ColorValue{23.65} & \ColorValue{14.23} & \ColorValue{17.43} & \ColorValue{16.88} 
& \ColorValue{5.18} & \ColorValue{27.97} & \ColorValue{45.44} & \ColorValue{48.12} 
& \ColorValue{4.31} & \ColorValue{8.51} & \ColorValue{8.79} & \ColorValue{58.04} 
& {\textbf{6}} \ColorValue{23.21}\\
\midrule

{MoELoRA}
& \ColorValue{7.13} & \ColorValue{1.98} & \ColorValue{1.93} & \ColorValue{34.74} 
& \ColorValue{0.19} & \ColorValue{1.75} & \ColorValue{2.05} & \ColorValue{29.24} 
& \ua{1.18} & \ColorValue{3.50} & \ColorValue{3.38} & \ColorValue{14.98} 
& {\textbf{\underline{2}}} \ColorValue{8.31}\\
\bottomrule
\end{tabular}
}

\label{table:benchmark_test}
\end{table*}
% \vspace{-20pt}



% The results of the fine-grained task of the benchmark are shown in Appendix~\ref{appendix:Q3_benchmark}.
